A Framework for Realistic Simulation of Daily Human Activity

For social robots like Astro which interact with and adapt to the daily movements of users within the home, realistic simulation of human activity is needed for feature development and testing. This paper presents a framework for simulating daily human activity patterns in home environments at scale, supporting manual configurability of different personas or activity patterns, variation of activity timings, and testing on multiple home layouts. We introduce a method for specifying day-to-day variation in schedules and present a bidirectional constraint propagation algorithm for generating schedules from templates. We validate the expressive power of our framework through a use case scenario analysis and demonstrate that our method can be used to generate data closely resembling human behavior from three public datasets and a self-collected dataset. Our contribution supports systematic testing of social robot behaviors at scale, enables procedural generation of synthetic datasets of human movement in different households, and can help minimize bias in training data, leading to more robust and effective robots for home environments.

==> backup.tex <==
\section{Abstract}
% To benefit from the capabilities of
Social robots such as Astro, to autonomously navigate around people in the home, need to understand human motion in various households over long periods of deployment. However, it is
difficult and impractical to gather this kind of training data -- in the wild --  directly from real people in their natural environment. Further, it is challenging to do so at scale.
% as we need large-scale training data, and 
A practical solution to this is the simulation of human motion. 
% Personal assistant robots in homes, offices, or hospitals can improve their interactions with people by understanding their surrounding environment patterns, including the users.
% For improved interactions in the household environment, simulation of human behavior and patterns over long periods is necessary. 
Existing approaches for human simulation work well in  generating probabilistic human motion patterns referred to as activity programs over multi-step tasks. However, these simulators do not focus on analyzing or generating realistic and long-term human movement patterns over days and/or weeks. We introduce a configurable human  motion generation algorithm that produces a varying schedule for daily human activity giving a template for human personas. We use a bidirectional constraint propagation approach to produce custom-tailored schedules. Our algorithm allows researchers to generate synthetic datasets of human movement inside different households procedurally, enabling training and testing of various movement understanding models. We further showcase how our generated synthetic dataset closely resembles real-life datasets of human movement in households. \iinote{Add statistics}

\section{FromIntroduction}
, \hl{such as finding a user in another room, choosing a path to stay out of people's way, or choosing to hang out in spaces where people are likely to be found}

However, simulation of daily activities in a realistic way is not straightforward, as daily activities include both structured and random components and depend on many social and contextual factors which vary from user to user. This paper presents a framework based on handcrafted schedule templates for simulating daily life activities and the resultant movement of humans around the home.

Our work aims to scalably generate simulated human motion data for varying household environments, while providing designers with the ability to configure the simulated users to emulate a variety of lifestyle patterns representing a range of age, work, and living situations. 

\section{Introduction}
% The first paragraph should generally describe the problem, focusing on the problem, what it is, and why it is important.  

% The characterization of people’s life has become an active area of research with the increasing availability of wearable sensors \cite{lara2012survey}. 
The advancement of navigational capabilities for commercial robot products requires the robot to build situational awareness of human users in the environment. 

For feature development and testing of robot behaviors which depend on spatial interaction with users or prediction of their locations, it is necessary to be able to reliably simulate human movement throughout the home. However, doing so in a realistic way can be very difficult, as daily activities include both structured and random components and depend on many social and contextual factors which vary from user to user. 

This paper presents an initial version of a framework for simulating daily life activities and the resultant movement of humans around the home. It was created for feature development and testing of the Amazon Astro robot (Fig. \ref{fig:astro}) in a Gazebo simulation environment.

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{images/astro.png}
    \includegraphics[width=0.375\linewidth]{images/gazebo.png}
    \caption{Left: Amazon's Astro robot.  Right: Gazebo-based simulation used in feature development and testing for Astro.}
    \label{fig:astro}
\end{figure}

However, the collection and annotation of long-term datasets that produce rich annotations of human motion in the wild  are challenging in terms of resources available. Further, extending such a data collection to various households is not scalable. Developing tools to simulate human behavior patterns over long periods is highly relevant in such scenarios. Our work aims to design specifications and an underlying algorithm that procedurally generates synthetic datasets that closely resemble the available real-life datasets. The dataset generated through our algorithm can help significantly improve human-robot interaction. Such datasets can enable the robots to autonomously build situational awareness by training on our synthetically generated datasets and develop autonomous behaviors for a consumer robot to hang out near people in the home.
% enable the robot help the development of algorithms that attempt to understand human behavior - the routine of activities of daily living or attempt to develop autonomous behaviors for a consumer robot to hang out near people in the home
% Our alimprove human-robot interaction by enabling the robot to build situational awareness by training on our synthetically generated datasets.

% outine, defined as the usual things that a person does daily, helps describe the individuals’ lifestyle.The characterization of people’s life has become an active area of research with the increasing availability of wearable sensors [25]. 
% The discovery of Routine and Non-Routine days from egocentric photo-streams is an important step for several applications, such as: self-awareness i.e. how does my daily life look like?; monitoring patients or assistance of elderly people (it is essential to know the person’s common behaviour and Routine) [9]; or, for memory enhancement and rehabilitation, which benefits from structuring the photo-stream into Routine and Non-Routine to easily find important events used in memory reminiscence therapy and interventions [28].


% The second paragraph should briefly describe related approaches and why they do not solve the problem.  
Over the past decade, the existing datasets for indoor human activity have been insufficient for developing autonomous behaviors for personal assistant robots, especially in an industrial setting.
\cite{lee2023developing}. The existing datasets do not capture the spatial and temporal information of the household humans' activities over long periods. They either contain annotations of low-level actions such as lying, standing sitting over minute-long samples.  Moreover, those datasets that do capture the long-term behaviors of the human containing high-level activities such as sleeping and eating fail to capture information on the whereabouts of the human inside the household. \iinote{insert ref of datasets}

Recent research introduced approaches for human simulation such as virtual home \cite{https://doi.org/10.48550/arxiv.1806.07011} and Alfred \cite{ALFRED20}. These work well in  generating probabilistic human motion patterns referred to as activity programs over multi-step tasks. However, these simulators do not focus on analyzing or generating realistic and long-term human movement patterns over days and/or weeks. These methods do not capture the realistic transition between socially meaningful activities and the time and location of executing an activity.

Manual generation of daily human activities over time is laborious, time-consuming, and would lack realism. Designing a framework that generates synthetic datasets for long-term patterns of realistic daily human activity is challenging. For a roboticist, such a dataset will be useful for training their models if it captures human schedules that vary according to the different human personas and the time of the week. Further, it should be easily usable, modifiable, and tunable by researchers through the configuration files, allowing the generation of application-specific datasets.
\iinote{Why is this challenging}
To our knowledge, there has not been a unified framework that generates datasets of varying and configurable schedules of humans. 

% The next few paragraphs should describe our technical approach to solving the problem.  The last paragraph should describe the evaluation and how we show that we have solved it.   I like to have a figure on the first page of the paper (Figure 1) that summarizes or shows what the robot can do that it couldn’t do before.  This figure is often the first thing reviewers see, and should show the “impressive result” of the paper visually, often a storyboard of the video.


The main contribution of our work is a novel formulation that generates configurable and variable schedules for daily human activity, given a template for human profiles. Our algorithm performs  iterative bidirectional constraint propagation to produce custom-tailored schedules. Our algorithm assumes access to a list of predefined human personas, including but not limited to elderly, employed adults, and lazy teenagers. It also assumes access to configuration files, such as schedule templates provided by the robotics engineers/designers, and includes. Given these configuration files, our algorithm performs bidirectional lookahead over the schedule template to 1) resolve conflicts that might exist in the template for overlapping activities. , 2) generates variation in the start/end times of activities based on the template provided, and 3) enables simulation of  motion over labeled locations in the household e.g., human moving around the kitchen for meal prep.
\iinote{Add: 2) ensures that the activities have no time gap by applying constraints to adjacent activities?}

We evaluate the usefulness of our method by measuring the similarity between our generated synthetic dataset with the publicly available long-term dataset \cite{vaizman2017recognizing}. Add: We perform an ablation study of our algorithm and compare the generated datasets to our method.  For comparison, we use the following metrics: \iinote{abc}. Our results show that our generated synthetic datasets are able to produce activities over \iinote{x} weeks of data and are \iinote{x\%} closer to UCSD.

% RELATED WORK

\subsection{Datasets for modeling Human Motion}
There exist datasets that capture human motion and activity patterns in indoor environments \cite{minne2019experimental, anguita2012human, shiwei_fang_2020_3882104, andrey_rudenko_2019_3405915}. However, most datasets do not capture human motion over long periods. They only capture short-term clips of activity useful for activity recognition but not for enabling autonomous behaviors in the long-term deployed robots. UCSD Dataset is the large-scale publically available dataset most relevant to our work \cite{vaizman2017recognizing}. It captures over 300k examples (minutes) from 60 users. Further, this dataset was collected from users engaged in their regular natural behavior. It also contains annotations are combinations of high-level activity labels from an extensive vocabulary.
% From every user it has thousands of examples, typically taken in intervals of 1 minute (but not necessarily in one long sequence, there are time gaps).
The ground truth n from the UCSD dataset is used to evaluate our human schedule generation algorithm. 
Other relevant work is by \citet{vintr2019spatio}. They gather a large dataset from a robot deployed in care homes and present a method that aims to model the periodic temporal patterns of people present over long periods, which are based on the routines and habits of people. However, this dataset only captures the detections of the people 
 and does not associate it with high-level activity.
 
 Other relevant datasets include as follows:
\citet{tran2017robots} deployed robot in-home care for five days. For their work, they possible schedules of the elderly, as shown in Fig. \ref{fig:elderly_schedule}. We compare our generate dataset with this reference human data, in terms of similarity
\citet{inproceedings} deployed robots at home for 63 days but only collected questionnaire and interview data for measuring acceptance.
\cite{hao2021invariant} mentions five long-term datasets but all were collected in the control environment.
\citet{TalaveraMartínez2021} collects a long-term dataset for 7 users over a week and learns to classify the days as routine/non-routine from an Ego-centric photostream. This publicly available dataset also classifies human time into various high and low-level activities as shown in Fig. \ref{fig:similarity_matrix}.

\cite{patel2022proactive} released the HOMER dataset for Household Object Movements based on schedules provided by Mechanical Turks. We compare our synthetic HumanAI schedule to this dataset HumanAI schedules.


\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{images/elderly_schedule.png}
    \caption{Schedule of the elderly as captured by the \cite{tran2017robots}}
    \label{fig:elderly_schedule}
\end{figure}


\section{Algorithm}
\textbf{1. Solving Duration Constraints}
For each $s_i$, we update any uninitialized start and end times according to the duration of each activity. by applying the following conditional rules: Eq-\ref{eq:dur1} and Eq-\ref{eq:dur2}:

\begin{align}
    &s_i[t_s] \gets 
    s_i[t_e] - s_i[d], & \text{if } s_i[t_e] \neq NULL
\label{eq:dur1}
\end{align}
\vspace{-5mm}
\begin{align}
    &s_i[t_e] \gets  s_i[t_s] +  s_i[d], & \text{if } s_i[t_s] \neq NULL
\label{eq:dur2}
\end{align}


\textbf{3) Solving Adjacency constraints}
The next step is to update time constraints between adjacent activities. In our model, we do not allow gaps between activities, so the activities with uninitialized start times begin when the previous task ends, and activities with uninitialized end times conclude at the start times of the next activity (Eq-\ref{eq:adjacency1} and Eq-\ref{eq:adjacency2}). 

\begin{align}
    &s_{i}[t_e] \gets 
    s_{i+1}[t_s], & \text{if } s_i[t_e] \eq NULL
\label{eq:adjacency1}
\end{align}
\vspace{-5mm}
\begin{align}
    &s_i[t_s] \gets s_{i-1}[t_e] , & \text{if } s_i[t_s] \eq NULL
\label{eq:adjacency2}
\end{align}


% For each activity updated by 

\textbf{4) Solving Non-contiguous Time Conflicts }
% WLookahead rule is applied to 
The start and end times generated for activities by Eq-\ref{eq:adjacency1} and Eq-\ref{eq:adjacency2} need to be filtered further because 
activities $ACT' \subset ACT$ updated by Eq-\ref{eq:adjacency1} and Eq-\ref{eq:adjacency2} can 
have time conflicts with the 
the non-contiguous activities above/below the activities in $ACT'$. To resolve these conflicts, we maintain a queue of direction pointers $P$ for the activities in $ACT'$. For each activity $act' \in ACT'$ updated by Eq-\ref{eq:adjacency1}, time conflict can arise with activities next in the time series. Hence, the direction pointer for these activities points to activities after $act'$; hence $p'=+1$ where $p' \in P$. For each activity $act'' \in ACT'$ that is updated by Eq-\ref{eq:adjacency2}, time conflicts can arise with activities earlier in the time series; hence the associate direction pointer $p'' \in P$. points to activities before $a'$; hence $p=+1$.

% Now consider the starting time of activity in $a'$; $s_{i}[t_s]$, and the direction to look ahead is (p=-1). 
To resolve conflicts, for each activity in $ACT'$, say the ith activity in schedule template $t$, we iterate in the direction of the direction pointer until we find the next activity next $t_{j}$ with a filled end time/start time according to Eq-\ref{eq:lookahead1} and Eq-\ref{eq:lookahead2}. 
Say for the ith activity in $ACT'$, the next filled activity is at the jth index,
now if the relevant time variable of the jth activity -- start time according to Eq\ref{eq:lookahead1} and end time for Eq-\ref{eq:lookahead2} overlaps over the ith activity, then we update these times for the ith activity 
% $s_{i}[t_s]$ from the end time of the$s_{j}[t_e]$ 
as illustrated in Eq-\ref{eq:lookahead1} and Eq-\ref{eq:lookahead2}

\begin{align}
    &s_{i}[t_s] = 
    s_{j}[t_e], & \text{if } s_i[act] \in act' \textit{\& } p = -1 \textit{\&} \nonumber \\
    & & \hspace{-5mm} j<i \textit{ \& } s_{j}[t_e] \neq NULL
\label{eq:lookahead1}
\end{align}
\vspace{-5mm}

% Now consider the case where $t_{i}[e]$ of a', and the direction to look ahead is (p=+1). To resolve conflicts, we iterate over the schedule template $t$ in the direction of the direction pointer until we find the next activity next $t_{j}$ with a filled start time -- $t_{j}[s] \neq NULL$. Now if $t_{i}[e]$ > $t_{j}[s]$ that is the jth activity overlaps over the ith activity then we end the ith activity $t_{i}[e]$ at the start time of the$t_{j}[s]$ as illustrated in Eq-\ref{eq:lookahead2}

\begin{align}
    &t_{i}[e] = 
    t_{j}[s], & \text{if } s_i[act] \in act' \textit{\& } p = +1 \textit{\&} \nonumber \\
    & & \hspace{-5mm} j>i \textit{ \& } t_{j}[s] \neq NULL
\label{eq:lookahead2}
\end{align}
% \vspace{-5mm}

% \begin{align}
%     &s_i[t_e] =  s_{j}[t_s] , & \text{if } s_i[act] \in act' \& p == +1 \& j>i \& 
%     t_{j}[s] \neq NULL
% \label{eq:lookahead2}
% \end{align}


We continue applying methods for 1) solving duration constraints, 2) solving adjacency constraints, and 3) solving non-contiguous Time Conflicts until the direction pointer queue $P$ gets empty. Our algorithm guarantees that $P$ gets empty because every pointer iterates the schedule template once in the stored direction until it finds an activity with the relevant information (Eq-\ref{eq:lookahead1}, Eq-\ref{eq:lookahead2}) or reaches the end of the schedule, after which it is removed from the queue.

The pipeline so far ensures that none of the activities overlap, but there can still be the case where a time gap exists between the activities specified in the template $t$. So we iterate over the $t$ once last time for updating $t$ according to Eq-\ref{eq:fillgaps}

\begin{align}
    &s_i[t_e] =  t_{j}[s] , & \text{if } s_i[t_e] \neq t_{j}[s]  \&  j>i 
\label{eq:fillgaps}
\end{align}

==> notes.tex <==
\section{Notes on our approach}
% The schedule template $t \in T$ is specified by the designer and is a list containing timing information for N activities.
% Each element of the template $t_i$ can be represented as the following tuple $t_i =(act, s\_t, s\_var, dur, dur\_var)$ where the $act$ is chosen from $ACT$, and $s\_t$ is the starting time for the activity $act$, $s\_var$ is the variance that the human user can take for starting the activity, $dur$ is the duration that the human activity can span for, and $dur_var$ is the variance that the human user can add to the total length of the activity. There is no limit on the $N$ - the total number of activities to be executed by the human daily. Further, any $act \in ACT$ can be executed by the human as many times as specified by the designer. For example, humans can exercise both in the morning and evening. For each $t_i$, all of the variables can be left blank except for the $act$
% e.g., cooking activity in the kitchen and eating in the dining room.
% This is not strictly 1-1 - e.g. both breakfast and lunch actions can happen in the dining room.
 % set of activities, $P$ is a set of human personas, and $T$ is a schedule template with partial sequencing order between $ACT$. 
 % These configuration files were chosen and designed for extensibility and controllability for user-specific personas and floor-specific locations. 


 
% The input tuple includes $I = (ACT, P, T)$. 
% The schedule template $t \in T$ is specified by the designer and is a list containing timing information for N activities. Each element of the template $T_i$ can be represented as the following tuple $t_i =(act, s\_t, s\_var, dur, dur\_var)$ where the $act$ is chosen from $ACT$, and $s\_t$ is the starting time for the activity $act$, $s\_var$ is the variance that the human user can take for starting the activity, $dur$ is the duration that the human activity can span for, and $dur_var$ is the variance that the human user can add to the total length of the activity. 
% There is no limit on the $N$ - the total number of activities to be executed by the human daily. 
% Further, any $act \in ACT$ can be executed by the human as many times as specified by the designer. For example, humans can exercise both in the morning and evening. For each $t_i$, all of the variables can be left blank except for the $act$
% A one-to-one mapping exists between $t \in T$ and $p \in P$ where each human persona $p$ corresponds to a unique schedule template $t$. $ACT$ is a set of pre-defined activities that can be performed by the human user as a part of their daily routine.
% Activity Location Map: A mapping between activities to labeled locations in the household. 


% and $act$ can be repea
% sequencing logic between activities. in $T$, the designer specifies the order of daily activities for the human user. These activities are chosen from $ACT$. For each 
% possible but not all sequencing logic between activities (e.g., start, duration, and variance) 
% A one-to-one mapping exists between $S$ and $P$ where each human persona $p in P$ corresponds to a unique schedule template $s \in S$. 
% For our research, we assume that each activity $act \in ACT$ is associated with a unique location/region in the room for its execution, e.g., cooking activity is performed in the kitchen and eating is performed in the dining room.
% We define activities set $ACT$, schedule $S$ as ${act_0, act_1,....act_n}$ where each $act_i \in Activities$. 
% For each human persona $p in P$, there is associated with 1) a Schedule Template that includes possible but not all sequencing logic between activities (e.g., start, duration, and variance) and 2) an Activity Location Map: A mapping between activities to labeled locations in the household. 
% $ACT$ including the possible but not all sequencing logic between activities (e.g., start, duration, and variance).

==> our_approach-old.tex <==
\section{Our Approach}


\begin{figure}[thb]
    \centering
    \includegraphics[width=\linewidth]{images/system-diagram-1.png}
    \caption{Elements of the proposed simulation framework}
    \label{fig:system-diagram-1}
\end{figure}

The elements of our proposed framework are shown in Fig. \ref{fig:system-diagram-1}, A designer first creates a \textbf{schedule template} specifying a time sequence of abstracted activities for a simulated user's day, including optional time constraints and ranges of variability for start times and activity durations.  The \textbf{schedule generator} processes this template to generate a set of varying daily activity schedules.
To support simulation in different homes, several \textbf{environment models} are defined, each containing a  \textbf{navigational floorplan}, used for path planning in the simulator, and a corresponding \textbf{activity-to-location map} defining specific ($x,y$) coordinates for each activity. 
The generated schedules are executed by the \textbf{simulation engine} to move simulated users around the home according to their scheduled activities throughout the day, generating a diverse set of synthetic data scenarios containing day-to-day schedule variations and a variety of home environments.

Activities are mapped to specific locations in the home.  For example, $cooking \rightarrow kitchen$. For each floorplan, we require an ($x,y$) location to be defined for each activity, allowing the floorplans to be interchanged, so the same schedule template can be used in different home layouts.

As the path-planning and obstacle-avoidance aspects of the human motion simulator are not novel, we will focus on the schedule generation aspect in this work. In the following subsections, we discuss the technical contribution in detail.

\subsection{Problem Formulation}
This section will describe the schedule generation algorithm. Let $T$ denote a schedule template consisting of an ordered sequence of $n$ constraints, where $T=\{c_1, c_2, ..., c_n\}$, and each constraint $c_i = (a_i,t_{start}^i, v_{start}^i, d^i, v_d^i)$, containing an activity $a_i$, a start time $t_{start}^i$ with variability $v_{start}^i$, and duration $d^i$ with variability $v_d^i$. For each entry, $a_i$ is required, but $(t_{start}^i,v_{start}^i)$ may be defined or left empty, and $(d^i,v_d^i)$ may be defined or left empty.

Next, let $S$ denote a generated schedule consisting of an ordered sequence of $n$ entries, where $S=\{s_1, s_2, ... , s_n\}$, and each entry $s_i = (a_i, t_{start}^i,d^i, t_{end}^i)$, containing an activity $a_i$,  start time $t_{start}^i$, duration $d^i$, and end time $t_{end}^i$.

\subsection{Iterative Bi-directional Constraint Propagation}
Algorithm \ref{alg:schedule} describes our method for generating a concrete schedule instance $S$ based on a schedule template $ST$.

\textbf{1. Initializing Random Values} The first step is to initialize $S$ from the constraints provided by the designer in the template. In this step, random variation is added to ($t_{start}$, $d$) from uniform distributions bounded by the specified ranges ($\pm v_{start}$, $\pm v_d$). For each entry $s_i$, $t_{end}$ is initialized to $null$.

The next step is to iteratively populate any uninitialized start and end times in $S$ by alternating between two update steps: applying duration constraints, and applying adjacency constraints. Rules are also applied to eliminate gaps in the schedule and avoid time conflicts.

\begin{algorithm}
\caption{Schedule Generation Algorithm}
\label{alg:schedule}
\hspace*{\algorithmicindent} \textbf{Input} Schedule template $ST$ \\
\hspace*{\algorithmicindent} \textbf{Output} Schedule $S$
\begin{algorithmic}[1]
\Procedure{GenerateSchedule}{ST}
    \State Apply random initialization to activities}}
    \For{each constraint $c_i \in T$}
        \State $s_i[a] \gets c_i[a]$        \If{$\exists(c_i[t_{start}],c_i[v_{start}]$)}
            \State $\Delta t \gets \mathcal{U}(-c_i[v_{start}],c_i[v_{start}])$
            \State $s_i[t_{start}] \gets c_i[t_{start}] + \Delta t$
        \EndIf
        \If{$\exists(c_i[d],c_i[v_d]$)}
            \State $\Delta t \gets \mathcal{U}(-c_i[v_d],c_i[v_d])$
            \State $s_i[d] \gets c_i[d] + \Delta t$
        \EndIf
    \EndFor

    \Comment{\hl{Step 2: Iteratively propagate constraints in $S$}}

    \While {$\exists s_i \ni \nexists s_i[t_{start}] \lor \nexists s_i[t_{end}]$} 
        \For{each entry $s_i \in S$}
            \State $\Call{ApplyDurationConstraints}{s_i}$
        \EndFor
        \For{each entry $s_i \in S$}
            \State $\Call{ApplyAdjacencyConstraints}{s_i}$
        \EndFor
        \If{no entries were updated in either step}
            \State \Call{Fail}{$underconstrained$}
        \EndIf
    \EndWhile
\EndProcedure
\end{algorithmic}
\end{algorithm}

\textbf{2. Solving Duration Constraints} (Algorithm \ref{alg:duration})
Because $s_i[t_{start}] + s_i[d] = s_i[t_{end}]$, we can determine the end time of any $s_i$ which has start time and duration defined, or the start time for any $s_i$ with end time and duration defined. 

After each duration update, there may be a time conflict with an adjacent or non-contiguous activity (as there may be uninitialized schedule entries lying between two time-conflicted activities). Our algorithm looks ahead to identify these conflicts at the time a duration constraint is applied.

For example, if $s_i[t_{end}] > s_j[t_{start}] \ni j > i$, then we shorten $s_i$ to end at $s_j[t_{start}]$. Any activities between them will be reduced to zero length and effectively deleted.  This procedure is applied both forwards and backwards.

Arguably, such a conflict could be treated as a schedule resolution failure, but we considered it realistic to simulate a situation where a user ``didn't get around to something" and skipped some activities to meet an upcoming time constraint.

Uninitialized start and end times are updated in this way for all applicable $s_i$.

\begin{algorithm}
\caption{Solving duration constraints}
\label{alg:duration}
\begin{algorithmic}[1]
\Procedure{ApplyDurationConstraints}{$s_i$}
    \If{$\exists s_i[t_{start}] \land \exists s_i[d] \land \nexists s_i[t_{end}]$}
        \State $j=arg\,min\{s_j[t_{start}]$ where $j > i\}$
        \State $s_i[t_{end}] \gets \min{(s_i[t_{start}] + s_i[d], s_j[t_{start}])}$
    \ElsIf{$\nexists s_i[t_{start}] \land \exists s_i[d] \land \exists s_i[t_{end}]$}
        \State $j=arg\,max\{s_j[t_{end}]$ where $j < i\}$
        \State $s_i[t_{start}] \gets \max{(s_i[t_{end}] - s_i[d],s_j[t_{end}])}$
    \EndIf
\EndProcedure
\end{algorithmic}
\end{algorithm}

\textbf{3. Solving Adjacency Constraints} (Algorithm \ref{alg:adjacency})
The next step is to update time constraints between adjacent activities. \hl{Unlike the discrete activities recorded in the datasets, which often have gaps between them, activities in our model represent persistent spatial locations, so we do not allow gaps between activities. Activities with uninitialized start times are thus defined to begin when the previous task ends,} and activities with uninitialized end times conclude at the start time of the next activity. If a gap exists between two activities, the earlier activity is extended to end at the start time of the later activity.

\begin{algorithm}
\caption{Solving adjacency constraints}
\label{alg:adjacency}
\begin{algorithmic}[1]
\Procedure{ApplyAdjacencyConstraints}{$s_i$}
    \If{$\exists s_i[t_{end}] \land \exists s_{i+1}$}
        \If{$\nexists s_{i+1}[t_{start}]$}
            \State $s_{i+1}[t_{start}] \gets s_i[t_{end}]$
        \ElsIf{$s_{i+1}[t_{start}] > s_i[t_{end}]$}
            \State Extend current activity to fill gap
            \State $s_i[t_{end}] \gets s_{i+1}[t_{start}]$
        \ElsIf{$s_{i+1}[t_{start}] < s_i[t_{end}]$}
            \State \Call{Fail}{$overconstrained$}
        \EndIf
    \EndIf
    \If{$\exists s_i[t_{start}] \land \exists s_{i-1}$}
        \If{$\nexists s_{i-1}[t_{end}]$}
            \State $s_{i-1}[t_{end}] \gets s_i[t_{start}]$
        \ElsIf{$s_{i-1}[t_{end}] < s_i[t_{start}]$}
            \State Extend previous activity to fill gap
            \State $s_{i-1}[t_{end}] \gets s_i[t_{start}]$
        \ElsIf{$s_{i-1}[t_{end}] > s_i[t_{start}]$}
            \State \Call{Fail}{$overconstrained$}
        \EndIf
    \EndIf
\EndProcedure
\end{algorithmic}
\end{algorithm}

\textbf{4. Exit criteria}
The iteration of constraint resolution continues until there are no schedule entries left with unresolved start or end times, indicating success.

The algorithm can fail to meet this condition if the schedule template is underconstrained. Such cases can be detected if no updates have been made to the schedule after a round of applying both duration and adjacency constraints. In these cases, the algorithm fails and no schedule is produced.

In other cases, the schedule may be overconstrained.  That is, a time conflict between two schedule entries cannot be resolved by adjusting a single start or end time.  Rather than implementing complex logic to handle these cases, we chose to allow the algorithm to fail in these situations.

\subsection{Validation of Schedule Template}
Because failure of the system to generate a valid schedule would be problematic at run time, such as during automated testing, we provide a design-time tool that designers can use to validate the schedule templates they create. Our validation algorithm is able to identify the following errors:
\begin{itemize}
    \item Chronological errors in the template
    \item Under-constrained conditions where the time constraints are insufficient to define a complete schedule 
    \item Over-constrained conditions where overlapping activities result in unresolvable time conflicts 
\end{itemize}

Because the process of schedule generation incorporates randomness, our validation algorithm generates schedules at the minimum and maximum extremes of the variance ranges. If it can be confirmed that there are no overlapping activities or underconstrained situations given these boundary values, then the template is considered valid. These validation steps are especially important for preventing failures during automated operations like regression testing or generation of large-scale synthetic datasets of user schedules. 

\subsection{Integration with the robot simulator}
As indicated in Fig. \ref{fig:system-diagram-1}, the generated schedules were used as one input into Astro's simulator, along with a floorplan and a mapping of activities to locations.
The simulations were executed in a photo-realistic simulator integrated with Gazebo, with the human simulation module moving each user to the target destination using an A* path planner with local obstacle avoidance for their scheduled activities based on the simulation wall-clock time.

The resultant simulation can be used in two ways.  First, the simulator can be used online with the robot software, to test and evaluate robot behaviors executed in relation to the simulated user(s). Alternatively, the output can be captured as a rosbag and added to a test corpus for offline replay.




==> paper_strategy.tex <==
\section{Paper Strategy}
% \iinote{Can you please add the paper strategy from quip document here or as a separate pdf in the repo. You can add comments by using \dgnote{}}

\textbf{Motivation:}
Personal assistant robots in homes, offices, or even hospitals must understand their surrounding environment, including their users. For improved interactions with their users, the robot needs to understand the patterns and behaviors of the users over long periods.


\textbf{Novelty}
Existing approaches for human simulation such as virtual home \cite{https://doi.org/10.48550/arxiv.1806.07011} and Alfred \cite{ALFRED20} work well in probabilistically generating human motion patterns referred to as activity programs over multi-step tasks. However, these simulators do not focus on analyzing or generating realistic human movement patterns over days and/or weeks. 

\textbf{Our Approach}
We introduce a configurable schedule generation algorithm that produces a schedule for daily human activity. We use a bidirectional constraint propagation approach to produce custom-tailored schedules.

\textbf{Method of Validation:}
We compare the generated daily schedule of human with real-life datasets.
Potential comparison methods include:
\begin{itemize}
    \item Comparison of the histogram of activity durations as shown in Fig-\label{fig:2}. We can use metrics like the correlation coefficient that generates a number between [0,1] defining correlation/similarity between histogram - a higher number means more correlation There are other histograms comparison metrics available at \url{https://docs.opencv.org/3.4/d8/dc8/tutorial_histogram_comparison.html} 
    \item  Comparison of the routine matrix as shown in Fig-\label{fig:1}
\end{itemize}



\begin{figure}[]
    \centering
    \includegraphics[width=0.8\linewidth]{images/unnamed.png}
    \caption{Histogram for durations Adopted from Internship work}
    \label{fig:2}
\end{figure}


\textbf{Hypothesis:}
Our generated behavior has a high correlation coefficient $>$ 0.5 than the real ones in terms of the histogram of durations and similarity matrix. This will show that our approach is best for recreating the kind of data in that dataset.

\textbf{Conclusion:}
Our procedurally generated schedule creates custom-tailored human motion data that can be used for various robotics learning applications such as obstacle avoidance,  learning state estimators for tasks, human schedule/activity recognition, or personalized interactions.

\textbf{Meeting Notes:}

\textbf{Todos [November,9th, 2022]:}
\begin{itemize}
    \item Ifrah -  Email authors for Public dataset
    \item Ifrah - Process and generate the durations over time graph for activities of the real-world dataset
    \item Ifrah - Structure the paper layout pages [intro+related] 
    \item Dylan+Sid - Figure how to generate more data in simulation 
\end{itemize}

\textbf{Todos [January, 2023]:}
\begin{itemize}
    \item Ifrah - Make a schedule for our paper
    \item Ifrah - Process and generate the durations over time graph for activities of the real-world dataset UCSD
    \item Ifrah - Structure the paper layout pages [abstract+intro+related] 
\end{itemize}

\textbf{Todos [Feb 17, 2023]:}
\\ Agenda
\begin{itemize}
    \item Discuss about Amazon sample data
    \item Show the labels of the dataset
    \item Show visualization
    \item UCSD's location granularity is at home, workplace/gym
    \item [sid] Visualization of Human-AI
    \item [sid] Support multiple human
    \item [motivation] get the robot out in the real world
    \item learning a template from reference data
    \item [sid, Dylan] learning template
    % \item []
\end{itemize}


1. Reference dataset:
     - UCSD: activity+poses(macro) simulating dataset
     - Long-Term Activity Recognition from Wristwatch Accelerometer Data. Sensors 2014,
     - care home environment
     - kerui dataset
     - STRANDS (weeks/months): focus
     - format of the datset (base UCSD)

 2. Synthetic Data
   - Appropriate schedule template, survey the team and ask for sample data

   - two direction:
        - learning a template from reference data
        - randomize the activities

        - this is possible to do
        - repeatable method works.

3. Multiple Metrics 
    - Visualization
    - Comparison
    -


\textbf{Todos [March 7, 2023]:}
\\ Agenda
\begin{itemize}
    \item Kerui's dataset and a common format for UCSD
    \item Discuss visualization and the labels of the dataset
    \item Ifrah: Find baseline for Human movement generation over long periods of time
    \item Ifrah: looks for dataset other than UCSD. Emailed one.
    \item Ifrah: discuss schedule template of elderly shown above and of another dataset \url{ https://figshare.com/articles/dataset/Long_term_activity_recognition_from_watch_accelerometer_data/1029775}.
    \item  dylan showed metric visualization
    \item no learning schedule template in the dataset. Hand-coded the template
    \item realistic and controllable, testing corner cases. Hand-tune does not capture all from data
    \item Design tool - four use-cases, case study expressive power to describe different schedules. The designer can tune the schedule.
    \item 2nd evaluation, cool to fit data. Is it expressive
    \item baseline  - Random motion  - follow the histogram distribution.
    \item future work switch the order qualitative
    \item motivate our algorithm
    
\end{itemize} 

Todos:
\begin{itemize}
    \item Sid: Support multiple humans
    \item [motivation] get the robot out in the real world
    \item Kerui to reformat the Pozyx data into the same format as the HumanAI schedules.  
    \item Dylan comparison code to measure similarity between schedules, and 
    \item Sid would perform the actual fit of the templates to the training data and output some example HumanAI schedules from his generated template.  
\end{itemize}

Three-pronged effort:  \\
1. Reference dataset: \\
     - [ifrah] UCSD: activity+poses(macro) simulating dataset \\
     - Long-Term Activity Recognition from Wristwatch Accelerometer Data. Sensors 2014, \\
     - care home environment \\
     - [Kerui] Kerui dataset \\
     - format of the dataset (base UCSD) \\

 2. [Sid] Synthetic Data \\
   - Appropriate schedule template, survey the team and ask for sample data \\

   - two directions: \\
        chosen: \\
        - learning a template from reference data \\
        - randomize the activities \\

        ignored this: \\
        - this is possible to do\\
        - repeatable method works.\\

3. [Dylan] Multiple Metrics  \\
    - Visualization \\
    - Comparison \\
 

March 8th,2023
Previous Meeting Todos:
\begin{itemize}
    \item Dylan will lead the visualization and comparison.
    \item Kerui will add a section for the Pozyx dataset and consider converting the UCSD dataset into the format Dylan requires. 
    \item Sid will visualize the time series schedule from the dataset.
    \item Ifrah will continue paper writing.- handcrafted adjustment to the data
    activity location synonmounis
\end{itemize}

Agenda
\begin{itemize}
    \item 
\end{itemize}








\newpage

